Global Convergence of Gradient Descent for Asymmetric Low-Rank Matrix Factorization

We study the asymmetric low-rank factorization problem: \[\min_{\mathbf{U} \in \mathbb{R}^{m \times d}, \mathbf{V} \in \mathbb{R}^{n \times d}} \frac{1}{2}\|\mathbf{U}\mathbf{V}^\top -\mathbf{\Sigma}\|_F^2\] where $\mathbf{\Sigma}$ is a given matrix of size $m \times n$ and rank $d$. This is a canonical problem that admits two difficulties in optimization: 1) non-convexity and 2) non-smoothness (due to unbalancedness of $\mathbf{U}$ and $\mathbf{V}$). This is also a prototype for more complex problems such as asymmetric matrix sensing and matrix completion. Despite being non-convex and non-smooth, it has been observed empirically that the randomly initialized gradient descent algorithm can solve this problem in polynomial time. Existing theories to explain this phenomenon all require artificial modifications of the algorithm, such as adding noise in each iteration and adding a balancing regularizer to balance the $\mathbf{U}$ and $\mathbf{V}$. This paper presents the first proof that shows randomly initialized gradient descent converges to a global minimum of the asymmetric low-rank factorization problem with a polynomial rate. For the proof, we develop 1) a new symmetrization technique to capture the magnitudes of the symmetry and asymmetry, and 2) a quantitative perturbation analysis to approximate matrix derivatives. We believe both are useful for other related non-convex problems.

==> theorems/proof_PD_range.tex <==
\begin{proof}[Proof of lemma \ref{lemm:PD range}]
When $d=1$, it is trivial.

When $d\geq2$, we can assume without loss of generality that $\xi=(1, 0, \cdots, 0)^\top$. If $d=2$, we assume that $\Sigma'=\left[\begin{matrix}
p & q\\
q & r
\end{matrix}
\right]$. Then $\sigma_d I\preceq \Sigma'\preceq \sigma_1 I$ is equivalent to three conditions below.
\begin{itemize}
    \item $\sigma_d\leq p, r\leq\sigma_1$;
    \item $(p-\sigma_d)(r-\sigma_d)\geq q^2$;
    \item and finally $(p-\sigma_1)(r-\sigma_1)\geq q^2$.
\end{itemize}
The necessity is obvious. For the sufficiency, we can conclude from that first condition that at least one eigenvalue of $\Sigma'$ is larger than $\sigma_d$, and at least one eigenvalue of $\Sigma'$ is smaller than $\sigma_1$. Then the second condition implies that once an eigenvalue is larger than $\sigma_d$, then all the eigenvalues are larger than $\sigma_d$. And similarly, condition 3 implies that all eigenvalues are smaller than $\sigma_1$. Hence, sufficiency follows.

Hence, we have $q^2\leq \min\{(p-\sigma_d)(r-\sigma_d), (p-\sigma_1)(r-\sigma_1)\}\leq (p-\sigma_d)(\sigma_1-p)$. Then $\left(p-\frac{\sigma_1+\sigma_d}{2}\right)^2+q^2\leq\left(\frac{\sigma_1-\sigma_d}{2}\right)^2$.

For the case of $d\geq 3$, we assume that $\Sigma'=\left[\begin{matrix}
p & q^\top\\
q & R
\end{matrix}
\right]$, where $q\in\mathbb{R}^{d-1}$ and $R\in\mathbb{R}^{(d-1)\times(d-1)}$. Then there exists a unitary matrix $\Phi$ such that $q^\top \Phi = (\|q\|_2, 0, \cdots, 0)$. Then we have
\begin{eqnarray}
\Sigma''\equiv\left[
\begin{matrix}
1 & 0\\
0 & \Phi^\top
\end{matrix}
\right]
\left[\begin{matrix}
p & q^\top\\
q & R
\end{matrix}
\right]
\left[
\begin{matrix}
1 & 0\\
0 & \Phi
\end{matrix}
\right] = 
\left[\begin{matrix}
p & q^\top\Phi\\
\Phi^\top q & \Phi^\top R\Phi.
\end{matrix}
\right]\notag
\end{eqnarray}

Because $\Sigma''$ is itself a matrix whose eigenvalues are lower and upper bounded by $\sigma_d$ and $\sigma_1$ respectively, we have the left-upper $2\times 2$ matrix also satisfies this condition. Hence, by the case of $d=2$, we have $\left(p-\frac{\sigma_1+\sigma_d}{2}\right)^2+\|q\|_2^2\leq\left(\frac{\sigma_1-\sigma_d}{2}\right)^2$. The sufficiency is also obvious, and the construction is simple.
\end{proof}

==> theorems/proof_dynamic_P2.tex <==
\begin{proof}
Similarly, we can expand the expression of $P'$ and split it in the following terms.
\begin{eqnarray}
\sigma_1(P')&\leq&\sigma_1\left(\beta P + 2\eta P^2 + \eta^2 P^3\right) + \sigma_1\left((1-\beta)P - \eta\Sigma P - \eta P\Sigma + \frac{\eta^2}{1-\beta}\Sigma P\Sigma\right)\notag\\
&& + \eta^2\sigma_1\left(-\frac{\beta}{1-\beta}\Sigma P\Sigma - \Sigma PP - PP\Sigma\right).\notag
\end{eqnarray}

For the first term $\beta P + 2\eta P^2 + \eta^2 P^3$, its singular values are $\beta p_i + 2\eta p_i^2 + \eta^2 p_i^3$ since $P$ is commutable with itself, where $p_i$ is the $i^{\text{th}}$ largest singular value of $P$. By the assumptions $|p_i|\leq \sigma_1$ and $\eta\leq\frac{\beta}{8\sigma_1}$, we see the largest singular value of $\beta P + 2\eta P^2 + \eta^2 P^3$ is exactly $\beta p + 2\eta p^2 + \eta^2 p^3$.

For the second term, it can be rewritten as
$$(1-\beta)P - \eta\Sigma P - \eta P\Sigma + \frac{\eta^2}{1-\beta}\Sigma P\Sigma \equiv \left(\sqrt{1-\beta}I-\frac{\eta}{\sqrt{1-\beta}}\Sigma\right)P\left(\sqrt{1-\beta}I-\frac{\eta}{\sqrt{1-\beta}}\Sigma\right).$$
Hence, the maximal singular value can be upper bounded by $\left(\sqrt{1-\beta}-\frac{\eta\sigma_d}{\sqrt{1-\beta}}\right)^2p$.

Finally, the last term can be upper bounded by $\eta^2\sigma_1\left(-\frac{\beta}{1-\beta}\Sigma P\Sigma - \Sigma PP - PP\Sigma\right)\leq \frac{2+\beta}{1-\beta}\eta^2\sigma_1^3$. Summing up all three terms and we get that when $p\leq0$,
\begin{eqnarray}
p'&\leq&\left(\beta p + 2\eta p^2 + \eta^2 p^3\right) + \left(\sqrt{1-\beta}-\frac{\eta\sigma_d}{\sqrt{1-\beta}}\right)^2p + \frac{2+\beta}{1-\beta}\eta^2\sigma_1^3\notag\\
&=& (1-\eta(\sigma_d - p))^2p + \frac{\beta\sigma_d^2}{1-\beta}\eta^2 p + 2\sigma_d\eta^2 p^2 + \frac{2+\beta}{1-\beta}\sigma_1^3\eta^2\notag\\
&\leq& (1-\eta(\sigma_d - p))^2p + \frac{2+\beta}{1-\beta}\sigma_1^3\eta^2.\notag
\end{eqnarray}
\end{proof}
